A Hybrid RAG System with Comprehensive Enhancement on Complex Reasoning

Retrieval-augmented generation (RAG) is a framework enabling large language models (LLMs) to enhance their accuracy and reduce hallucinations by integrating external knowledge bases. In this paper, we introduce a hybrid RAG system enhanced through a comprehensive suite of optimizations that significantly improve retrieval quality, augment reasoning capabilities, and refine numerical computation ability. We refined the text chunks and tables in web pages, added attribute predictors to reduce hallucinations, conducted LLM Knowledge Extractor and Knowledge Graph Extractor, and finally built a reasoning strategy with all the references. We evaluated our system on the CRAG dataset through the Meta CRAG KDD Cup 2024 Competition. Both the local and online evaluations demonstrate that our system significantly enhances complex reasoning capabilities. In local evaluations, we have significantly improved accuracy and reduced error rates compared to the baseline model, achieving a notable increase in scores. In the meanwhile, we have attained outstanding results in online assessments, demonstrating the performance and generalization capabilities of the proposed system. The source code for our system is released in \url{https://gitlab.aicrowd.com/shizueyy/crag-new}.

==> sections/related.tex <==
\section{Related Works}\label{sec:related-work}
There are several techniques to solve the problems mentioned before. For example, formal verification can help to reduce hallucination and output the verified reasoning process\cite{xiong2023trigo,wang2023dt,liu2023fimo}. Moreover, there are some efficient training methods\cite{shen2022palt,pan2023reusing-mango-nips,pan2024preparing-apollo-aaai} that can help the model adapt to domain-specific knowledge.
Given its significant potential to mitigate the well-known issue of hallucination and enhance domain-specific knowledge integration, retrieval-augmented generation has recently garnered substantial research attention within the scientific community.
While numerous approaches have been proposed in the literature, the majority are tailored to address specific issues within a limited range of scenarios, making them unsuitable for direct application to CRAG tasks.
We present a compilation of recent research to highlight the diverse design choices within the broader RAG research community.
Some of the works included in this compilation are effective for specific CRAG tasks and have been integrated into our system, while others are not.
Drawing inspiration from recent advancements in the field, we have developed a novel design that integrates multiple strategies.

We built upon previous research \cite{huang2024survey, gao2023retrieval, wu2024retrievalaugmentedgenerationnaturallanguage,yuan2024measuring} to structure the conventional RAG workflow into four phases: pre-retrieval, retrieval, post-retrieval, and generation.

\subsection{Pre-retrieval}

The pre-retrieval phase involves indexing, query manipulation, and data modification. That is, compiling and indexing external knowledge sources to enhance the efficiency of subsequent searching execution, refining the query to better match the external data distribution and modifying data sources to create a coherent representation that encapsulates relevant knowledge for further reasoning.

\textbf{Indexing:} Given that external knowledge sources --- specifically, the limited web pages in CRAG tasks --- are accessible solely during the inference stage and are tailored to each user query, pre-indexing these sources would offer little performance enhancement in CRAG tasks.
Nevertheless, the design choices are closely related to the retrieval phase, warranting their discussion here.
Text indexing has emerged as a prominent area of research within the field of data mining, leading to the development of numerous methodologies.
Traditional indexing methods include the inverted index \cite{zobel2006inverted}, suffix tree \cite{mccreight1976space}, and term frequency-inverse document frequency (TF-IDF) index \cite{sparck1972statistical}.
These indexing methods utilize term frequency so that they may neglect the semantic information inherent in the text.
Recent indexing methods employ language models such as BERT \cite{devlin2018bert} and Sentence-T5 \cite{ni2021sentence} to encode text into vectors within latent space.
These vectors are used to construct vector indexes \cite{douze2024faiss} that enhance similarity search through techniques including product quantization (PQ) \cite{jegou2010product}, Hierarchical Navigable Small World (HNSW) \cite{malkov2018efficient}, and Navigating Spreading-out Graph (NSG) \cite{fu2017fast}.

\textbf{Query Manipulation:} The manipulation algorithms discussed below contribute to developing an improved metric for evaluating the similarity between user queries and external data.
It is desirable to formulate a fully specified, context-independent query that effectively articulates user intent and aligns with the distribution of external knowledge sources.
Query manipulation, also known as query rewriting, serves multiple purposes.
It can involve reformulating questions to enhance clarity, simplifying language, or tailoring the question for various contexts or audiences.
Early research primarily utilizes an n-gram language model derived from hundreds of millions of web search sessions \cite{jansen2009patterns} or employs a pointer-generator network to improve referring expression resolution.
Recent studies have leveraged the few-shot or zero-shot learning capabilities of language models that utilize a small set of manually created rewriting labels \cite{yu2020few, yu2022generate}.
The versatile capabilities of LLMs enhance the flexibility of query manipulation.
In contrast to traditional query rewriting, which follows a ``query in, query out'' format, recent query manipulation approaches utilizing LLMs allow for ``query in, passage out'' approaches \cite{yu2022generate, ma2023query}.

\textbf{Data Modification:} Data extracted from original external knowledge sources may contain elements that are not conducive to the reasoning process of LLMs, such as redundant HTML tags found in web pages.
Therefore, data modification is necessary to transform the original data into a more knowledge-rich format that is suitable for further reasoning.
However, these processes are closely linked to the format and distribution of external knowledge sources and often involve tedious text normalization procedures that are largely unrelated to the reasoning process, including tokenization, stemming, and the removal of stop words.
Prior research has examined the use of substrings as document identifiers to improve search capabilities \cite{bevilacqua2022autoregressive}, as well as the application of LLMs to recite one or more relevant passages from their internal memory \cite{sunrecitation}.

\subsection{Retrieval}

The retrieval phase primarily involves searching for pertinent materials from external knowledge sources and ranking them according to their relevance to the user query.

\textbf{Search:} Searching for relevant documents efficiently from vast external knowledge sources, such as the entire Internet, can be exceedingly challenging.
However, in the context of CRAG tasks, a search engine and a mock API handle the search process for us.
The dataset provides a relatively small number of web pages (five candidates for Task 1 and Task 2, and fifty candidates for Task 3), thereby alleviating the challenges associated with effective searching.
Previous research on RAG that aims to retrieve local data typically employs local vector databases, such as Elasticsearch \cite{gormley2015elasticsearch}, or utilizes libraries like FAISS \cite{douze2024faiss} for efficient similarity search and vector clustering.
On the other hand, research focused on general-purpose RAG typically utilizes external web search engines directly; for instance, WebGPT \cite{nakano2021webgpt} employs the Bing API.

\textbf{Ranking:} The ranking metric establishes the priority of each document housed in external knowledge sources.
The metric used to evaluate the similarity between a potentially manipulated query and a document can be classified into two categories: sparse retrieval and dense retrieval. 
Sparse retrieval metrics, such as BM25 \cite{robertson2009probabilistic, izacard2021leveragingpassageretrievalgenerative} and Term Frequency–Inverse Document Frequency (TF-IDF) \cite{chen2017reading}, rely on word frequency, whereas dense retrieval metrics utilize embedded vector, including Euclidean distance \cite{khandelwal2019generalization}, cosine similarity \cite{juvekar2024cos}, and Dense Passage Retrieval (DPR) \cite{karpukhin2020dense, izacard2021leveragingpassageretrievalgenerative}.

\subsection{Post-retrieval}

The post-retrieval phase includes re-ranking and filtering, which further aligns the ranking to the user intent, refining the ranking results, and filtering out materials that are irrelevant to the querying topic.

\textbf{Re-ranking:} Although vector similarity-based document retrieval can be executed efficiently and effectively, including in parallel \cite{johnson2019billion, khattab2020colbert} or distributed systems \cite{echihabi2021new}, its capacity to reveal semantic relationships between queries and documents remains constrained \cite{steck2024cosine}.
This is where re-ranking becomes significant: typically bigger models, which offer greater accuracy but lower efficiency, can precisely reorder the limited set of documents retrieved.
The CRAG tasks assign the information retrieval function to external web search engines and knowledge graph mock APIs, yielding a streamlined selection of documents for each query.
In this context, the extraction of relevant information from a limited set of articles resembles a reordering process rather than traditional retrieval.
Some approaches \cite{glass2022re2g, ram2023context} embed the query-document pair in a single pass, facilitating cross-attention between sequences.
These approaches enhance the evaluation of mutual information between the texts.
Other studies employ large language models as few-shot annotators to generate data for training a cross-attention re-ranker \cite{dai2022promptagator}, or investigate the auto-regressive generation of re-ranking results to leverage inter-document relationships \cite{hofstatter2023fid}.

\textbf{Filtering:} Filtering seeks to remove redundant parts from the retrieval results, which may either be of poor quality or exhibit low relevance to the user query \cite{wang2023learning}.
Current studies employ large language models to evaluate the utility of retrieved information and to critique whether all verification-worthy statements are substantiated by the associated documents \cite{asai2023self, wang2024blendfilter}, or condense retrieved documents into a textual summary, thereby minimizing inference costs \cite{xu2023recomp}.

\subsection{Generation}

The curated reference materials are subsequently processed in the generation phase to produce the final results.
Additionally, various enhancement techniques and customizations can be applied to the same phrase.

\textbf{Enhancing:} Enhancing, also known as retrieval fusion, seeks to improve the performance of large language model generations by utilizing retrieved documents.
Typically, the retrieved documents are concatenated with the query in the expectation that the language models will generate coherent results based on the reference materials \cite{lewis2020retrieval, ram2023context, guu2020retrieval}.
Other methods utilize sophisticated prompt templates that integrate multiple pieces of information \cite{vu2023freshllmsrefreshinglargelanguage} or employ techniques such as context compression, summarization, and filtering to achieve more efficient inference \cite{arefeen2024leancontext, liu2023tcra, wang2023learning, xu2023recomp}.
Several studies have also investigated the integration of encoded retrieval vectors into input features \cite{izacard2021leveragingpassageretrievalgenerative, izacard2023atlas, singh2021end}.

\textbf{Customization:} During the customization process, it is crucial to meticulously refine the model's outputs to ensure alignment between the model's responses and the user's intended queries.
This refinement will result in final answers that are concise, informative, and well-formatted.
The customization strategy may vary significantly depending on the specific task requirements.
These approaches include generating reflection tokens for self-evaluation of the model's output \cite{asai2023self} and implementing a graph-text contrastive learning method to enhance the alignment between generated content and retrieved references\cite{kang2023knowledge}.



